Spin glasses, the quantum annealing, colloidal glasses and crystals: exploring complex free-energy landscapes

Glassy behavior is one of the main open problems in condensed matter physics. In this thesis, we approach the problem by studying spin-glasses and colloids, using several complementary strategies. From the point of view of model building, we propose a new model, the hypercube model, which is mean-field but defined in a metric space. We show that, also in Mean Field, the spin-glass non-equilibrium dynamics is a domain-growth process very similar to its three-dimensional counterpart. We also consider spin-glasses in three spatial dimensions, focusing on temperature chaos. Thanks to the low-temperature configurations equilibrated with Janus, we show that temperature chaos can be aptly described through a large-deviations functional. The finite-size scaling behavior can be predicted in details from this functional, including the pre-asymptotic regime where chaos is driven by rare events. We also address the problem of finding new, efficient algorithms to study glassy systems. In particular, in the context of the Quantum-Adiabatic algorithm we discuss strategies for bypassing the "first-order bottleneck". Our approach is successfully put to work on the p-spin ferromagnetic model. We also show how to use tethered Monte Carlo (a recent refinement of Umbrella Sampling) to handle problems with more than one order parameter, such as hard-spheres crystallization. We study the crystallization transition equilibrating the largest systems to date, and obtaining very accurate determinations of the coexistence pressure and the interfacial free-energy. We also show our efforts to characterize the solid phase in a system of soft spheres at very high polydispersity.

==> coloides.tex <==
\chapter{General Definitions \label{chap:intro-colloids}}


\section{Observables}
\subsection{Crystalline parameters}

The standard order parameter for modern crystallization studies is
$Q_6$~\cite{steinhardt:83,duijneveldt:92}, which is the $l=6$ instance
of
\begin{equation} 
Q_l \equiv \left( \frac{4 \pi}{2l +1} \sum_{m = -l}^{l} \left|
Q_{lm} \right|^2 \right)^{1/2}\,,
\end{equation}
where
\begin{equation}
Q_{lm} \equiv \frac{\sum_{i=1
  }^{N}\, q_{lm}(i)}{\sum_{i=1 }^{N} N_b(i)}\,,\quad q_{lm}(i) \equiv
\sum_{j=1}^{N_b(i)} Y_{lm}({\hat{\V{r}}_{ij}})\,.
\end{equation}
In the above expression, $Y_{lm}(\hat{\V{r}}_{ij})$ are the spherical
harmonics, while $\hat{\V{r}}_{ij}$ is the unit vector in the direction
joining particles $i$ and $j$, $\V{r_{ij}}=\V{r}_i-\V{r}_j$.  $N_b(i)$
represents the number of neighbors of the $i$th particle.
\footnote{Two particles $i$ and $j$ are considered neighbors iff
  $r_{ij}<1.5\ \sigma$. This choice ensures that we enclose only the
  first-neighbors shell in the FCC structure, for all the densities of
  interest here~\cite{seoane:12}.} It is important to note that, letting aside
the periodic boundary conditions for our simulation box, $Q_6$ is rotationally
invariant.  $Q_6$ is of order $1/\sqrt{N}$ in a fluid phase, whereas
$Q_6\approx0.574$ or $0.510$ in perfect FCC or BCC crystals, respectively. 
However, defective crystals have lesser values ($Q_6\approx 0.4$ is fairly
common).

Now, if one tries to perform a tethered computation, choosing $Q_6$ as order
parameter, it is soon discovered that it is almost imposible to form a FCC
crystal if the starting particle configuration is disordered. Instead, the
simulation gets stuck in helicoidal crystals, with a similar value of $Q_6$,
which are allowed by the periodic boundary conditions. The crystalline planes
for these helicoidal structures are misaligned with the simulation box.  Upon
reflection, one realizes that the problem lies in the rotational invariance of
$Q_6$. When a crystalline grain starts to nucleate from the fluid, which is
encouraged by the tethered algorithm for large $\hq$, we face the problem that
$Q_6$ conveys no information about the relative orientation of the growing
grain with respect to the simulation box. At some point, the misaligned
crystalline grain is large enough to hit itself through the periodic boundary
conditions, and it needs to contort itself to get some matching for the
crystalline planes.

The way out is in an order parameter with only cubic symmetry.  Such a
parameter was recently proposed~\cite{angioletti:10}:
\begin{equation}\label{eq:C}
C=\frac{2288}{79}\frac{\sum_{i=1}^{N} \sum_{j=1}^{N_b(i)}c_{\alpha}({\hat{\V{r}}_{ij}})}{\sum_{i=1 }^{N}N_b(i)}-\frac{64}{79} \,,
\end{equation}
where 
\begin{equation}
c_{\alpha}(\hat {\V{r}})=x^4y^4(1-z^4)+x^4z^4(1-y^4)+y^4z^4(1-x^4)\,.
\end{equation}
The expectation value for $C$ in the different phases is the following: $0.0$
in the fluid, $1.0$ in the ideal FCC crystal, perfectly aligned with the
simulation box, and $-0.26$ in the perfectly aligned ideal BCC.  The
difference with the quoted value in Ref.~\cite{angioletti:10} for the perfect
BCC crystal is in our smaller threshold for neighboring particles. Again, as
it happens for $\q$, we must expect lower $|C|$ values for defective
structures.

In fact, we find that tethered simulations with a single order parameter ($C$)
and large $\hat C$, equilibrate easily. One forms nice crystals even if the
starting particle configuration is disordered, and the Monte Carlo expectation
values turn out to be independent of the starting configuration, as they
should. 

However, not all is well. At some intermediate values of $\hat C$ the
simulation suffers from metastabilities. Heterogeneous states with a slab of
FCC crystal in a fluid matrix are degenerate with helicoidal crystals, that
fill most of the simulation box, but have a small value of $C$ because of
their missalignment. Fortunately, these two types of competing configurations
are clearly differentiated by $\q$, which is large for the helicoidal crystal,
but small for the crystalline slab surrounded by fluid. Therefore, the
combination of the two order parameters labels unambigously the intermediate states between the fluid and the FCC crystal.

